GossipGraD: Scalable Deep Learning using Gossip Communication based Asynchronous Gradient Descent

In this paper, we present GossipGraD - a gossip communication protocol based Stochastic Gradient Descent (SGD) algorithm for scaling Deep Learning (DL) algorithms on large-scale systems. The salient features of GossipGraD are: 1) reduction in overall communication complexity from {\Theta}(log(p)) for p compute nodes in well-studied SGD to O(1), 2) model diffusion such that compute nodes exchange their updates (gradients) indirectly after every log(p) steps, 3) rotation of communication partners for facilitating direct diffusion of gradients, 4) asynchronous distributed shuffle of samples during the feedforward phase in SGD to prevent over-fitting, 5) asynchronous communication of gradients for further reducing the communication cost of SGD and GossipGraD. We implement GossipGraD for GPU and CPU clusters and use NVIDIA GPUs (Pascal P100) connected with InfiniBand, and Intel Knights Landing (KNL) connected with Aries network. We evaluate GossipGraD using well-studied dataset ImageNet-1K (~250GB), and widely studied neural network topologies such as GoogLeNet and ResNet50 (current winner of ImageNet Large Scale Visualization Research Challenge (ILSVRC)). Our performance evaluation using both KNL and Pascal GPUs indicates that GossipGraD can achieve perfect efficiency for these datasets and their associated neural network topologies. Specifically, for ResNet50, GossipGraD is able to achieve ~100% compute efficiency using 128 NVIDIA Pascal P100 GPUs - while matching the top-1 classification accuracy published in literature.

==> Makefile <==
#
# $Id: Makefile 161 2007-11-30 07:19:52Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

.PHONY: all clean complete

tex_files = $(wildcard *.tex */*.tex */*/*.tex */*/*/*.tex)
bib_files = $(wildcard *.bib */*.bib */*/*.bib */*/*/*.bib)
eps_files = $(wildcard *.eps */*.eps */*/*.eps */*/*/*.eps)
epsi_files = $(wildcard *.epsi */*.epsi */*/*.epsi */*/*/*.epsi)
ps_files = $(wildcard */*.ps */*/*.ps */*/*/*.ps)

all: header.tex $(tex_files) $(bib_files)
	pdflatex header
	bibtex header
	pdflatex header
	pdflatex header

header: header.tex $(tex_files) $(bib_files)
	@if test "`which rubber `" != "" ; then \
		rubber -d header ; \
	else \
		pdflatex header | tee latex.out ; \
		if grep -q 'Warning: Citation.*undefined' latex.out; then \
			bibtex header; \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '^LaTeX Warning:.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex header | tee latex.out; \
		done ; \
		rm latex.out ; \
	fi

clean:
	find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
		\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
		\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
		\( -name '*.toc' -print \) | xargs rm -f; \
	rm -f header.dvi header.log header.pdf _region_* \
		summary.pdf cv_vishnu.pdf header.out


==> text/design.tex <==
\section{Solution Space}
\label{sec:design}
\subsection{Simple Data-parallel SGD}
Our proposed solution space for scaling SGD on distributed memory systems builds on 
a simple data-parallel approach.  We first replicate the complete network model 
and solver (connectivity, synapse weights, and initial conditions) across all
compute nodes so that each node has a complete copy of the model and solver. 
The data elements comprising each batch set are partitioned across the
compute nodes.  For each iteration, every node performs forward and backward
propagation calculations using its portion of the data elements comprising 
that iteration's batch.
Each node calculates its own gradient vector using the results from its 
subset of the batch data.  The locally-calculated gradient vectors from all 
nodes are averaged together and then copied back to node.  All nodes still
have the same initial starting synapse weights and solver conditions, and
all will use the same gradient vector for updating their synapse weights.  
After the update, all nodes will again share an identical (updated) model state.
This simple approach will generate the same results as a single-node 
implementation, and allows scaling up to a number of nodes equal to the number
of data elements in a batch.  For our tests, we implemented this baseline
distributed memory implementation on Linux machines equipped with Infiniband
networking cards, and performed the global gradient vector averaging with
an  MPI\_Allreduce MPI\_Sum operation, followed by local vector rescaling by
1/total number of nodes. 
  
\subsection{SGD within subgroups}
From that initial approach (which performs the same as a single-node system), 
we reduce the number of nodes that must communicate with each other
during each iteration in exchange for allowing a delay before each gradient's
update reaches all other nodes.
In the simple data parallel approach, performing the gradient vector average
across all nodes is effectively a reduction/broadcast operation
requiring $\log2{n}$ exchanges for each gradient vector element.
If we could subdivide our initial group of ($N$) nodes into k equally-sized
subgroups for each iteration (carefully reassigning the subgroup members
at each iteration to ensure good mixing), each averaging operation can be
reduced from $\log2{n}$ to $\log2{n/k}$ = $\log2{n}$ - $\log2{k}$ exchanges. 

While this approach necessitates introducing an additional averaging operation
before calculating gradients, for a sufficiently large number of small subgroups
it becomes worthwhile. 

Consider a set of 16 nodes performing the global gradient averaging using the
simple data-parallel approach as initially described above.
The global average requires $\log2{16}$ =4 send/receive operations for each 
vector element at each step.  Now consider that for calculating
the first batch, we divide those 16 nodes into two different subgroups 
of 8 nodes, where subgroup membership is assigned by the 0th bit of the 
node ID. (i.e. Group 0 contains nodes 0, 2,4,6,8,10,12,14 and Group 1 contains
nodes 1,3,5,7,9,11,13,15).  Each subgroup calculates and applies it's own
global average gradient vector j-> now the two groups have two different sets
of synapse weights.

For the second batch, we repartition the 16 nodes into 2 new subgroups defined
by the value of the next bit (bit 1) in the node ID, so that now Group 0 
contains nodes 0,1,4,5,8,9,12, and 13 and Group 1 contains nodes 2,3,6,7,10,11,14,
and 15.  Half the nodes within each of these new subgroups have a different set of 
synapse weights compared to the other half, so we must first average their
current synapse weights within (not across) each subgroup.  After this 
inital averaging, all the nodes in both subgroups will again share a common
set of synapse weights.  This state will be very close to the state that would
have been reached by the simple data-parallel model after the 1st batch gradient
updates were applied.  In the simple data-parallel model, a common set of synapse
weights was updated by applying a common gradient at all nodes.  That common
gradient is equal to the average of the two subgroup gradients. In our subgroup
model, exactly half the nodes in each subgroup had one subgroup gradient
applied and the other half had the other subgroup gradient applied. By averaging
the synapse weights of these two halves before doing forward/backward
propagation, both subgroups reach a set of synapse weights nearly identical 
to the synapse weights of the simple data-parallel model.

Each node within each subgroup calculates its local gradient vector based on
its subset of batch elements, and the nodes within each subgroup again
compute a subgroup (not global) average gradient vector, and then update
their weights.

At the beginning of the third batch, the nodes are repartitioned again
into 2 new subgroups defined by bit 2 of the node ID, so that the new
Group 0 contains 0,1,2,3,8,9,10,11 and Group 1 contains 4,5,6,7,12,13,14,15.
Each group first averages the synapse weight values for all nodes, and is
again at a state nearly identical to the simple data-parallel model after
it's second batch gradient updates were applied.  All nodes are have a
common value, and the process continues.

In this simple 2-subgroup example, we are actually doing more communication
than we would do with a global averaging, but it illustrates the basic 
concept of applying a partial gradient at one time, and then averaging
the synapse weights at a later time to bring in the effect from the 
skipped partial gradient.  For the moment, we are ignoring the 
solver state (e.g. momentum), although this could be averaged across the
nodes of each subgroup at the same time the synapse weights are averaged.
In practice, the additional convergence obtained from this averaging
is small relative to the cost of the additional communication step.

Our first design-space parameter is the degree to which we divide a given
number of nodes into subgroups.  If we have only 1 (sub)group, we are back
to the simple data-parallel baseline case.  At the most extreme, we have
$\log2{N-1}$ subgroups of 2 nodes each (assuming {\em N} is a power of 2), and it
requires $\log2{N}$ iterations to fully diffuse the effect of the first 
batch's gradient calculation to all nodes.

\subsection{Subgroup membership assignment}
The second design-space parameter is the means by which subgroup membership
is re-assigned at each iteration.  The simplest means of subgroup assignment
while ensuring good mixing of prior gradients' effects across nodes is to 
simple use the value of certain index bits at different positions within each
node's ID. To ensure optimal mixing, avoid (or at least minimize) the overlap
of index bit positions from one stage to the next. For instance, if we have
256 nodes (8 index bits), but want to 4 groups of 64 nodes each (2 bit 
positions determine group membership), we could use bits (0,1) for
the first stage, (2,3) for the second stage, (4,5) for the third stage,
and (6,7) for the fourth stage.  We would NOT want to repeat bits across 
adjacent stages (e.g. (0,1) for the first stage, (1,2) for the second stage,
(2,3) for the third stage, etc), nor would we want to repeat index bit usage
until all index bits have been used at least once.  Avoiding repeats and
overlaps is especially important for the earliest stages.  

This design-space dimension is also concerned with how the next set of 
set of subgroup memberships are assigned.  The degenerate case is simple:
repeat the same subgroup assignments.  For our 256 node/4 subgroup example,
iteration 5 would thus have the same assignments that iteration 1 had.
example).  Extending along this dimension, we can remap the true node ID
to an index ID used to assign subgroup membership using varying degrees
of complexity that range from simple increment (mod N) by a fixed
(ideally prime), by incrementing (or increasing prime) numbers,
or by a Fisher-Yates reshuffling based on a shared seed across all nodes.
The increased mixing by resequencing becomes more importance for larger
numbers of subgroups containing small numbers of nodes with small 
numbers of batch elements at each node. 


\subsection{Longer deferral for better communication/computation overlap}
The third design-space dimension is a variation of the first dimension.
For that first dimension, the number of nodes that must communicate 
with each other in each batch was reduced in exchange for longer delays
(number of iterations) before the full effect of each subgroup's
gradient calculations from a particular batch would reach and influence
all other nodes.  At it's maximal extent, nodes exchange data with
only one or two other nodes for each batch.  Our third design 
dimension allows greater overlap of communication with computation 
by deferring the averaging of synapse weights and gradient vectors
by one or more batches. This is our first really significant divergence
from the original data-parallel model.  Rather than calculating local 
gradients within a subgroup using a "current" set of synapse weights,
a node begins each batch by averaging its current synapse weights with
the synapse weights of the prior subgroup partner.
The node also averages it's previously-calculated gradient vector with
the prior subgroup partner's gradient vector and applies the average 
to the averaged synapse weights.  These updated, averaged synapse weights
are sent (non-blocking) to the current subgroup partner for it's use 
on the next batch.  Forward/backward propagation is run on the updated
synapse weights using the current batch data, and the resulting 
gradient vector is kept locally for the next iteration, and sent (nonblocking)
to the current subgroup partner for use on it's next batch.  
After the gradient sent is initiated, the current iteration is complete.
This deferred update can potentially be extended for more than one batch, or 
even alternated with a purely locally-applied batch, to maximize 
communication / computation overlap, at the expense of greater divergence 
across nodes.

\subsection{Periodic global averaging}
To correct these accumulating divergences, global averaging of the synapse
weights and solver momentum can be periodically performed.  The fourth 
design-space dimension is the frequency, or trigger basis, for which
these periodic global averages of synapse weights and solver momentum
occurs to minimize model divergence across the nodes.

\subsection{Model scaling across more than one node}
The fifth design-space dimension is orthogonal to the others and relates to 
distributing a single model instance across more than one compute node.
This would replace all instances of "node" in the above 4 dimensions with
a "model instance node" comprised of several compute nodes.  The total
number of nodes would scale by the degree by which the model could be distributed,
and the speed would scale by the relative performance of the multi-node model
compared to a single-node model; this would be highly dependent upon the 
actual neural network architecture being simulated.  Distribution of model
synapse weights across the nodes would decrease the communicate per compute node at 
each stage (compared to a single compute node model implementation), but may
still have enough latency that it won't overlap as cleanly with model node - to -
model node subgroup commmunication.  If necessary, an additional 1-batch delay 
could be added, so that the intra-node communication to calculate the 
forward/backward propagation loss using the model nodes' subset of the 
current batch data elements could be overlapped with the communication 
synapse weights and gradients between model nodes in the subgroup.






==> text/dist.tex <==
\section{Other Implementation Details}
\label{sec:impl}
The implementations evaluated in this paper focus on data parallelism
and the averaging of gradients across compute devices. This is achieved
using MPI and parallel I/O.

\subsection{Handling I/O}
The data parallelism is achieved by distributing datasets across compute
devices, partitioning them based on the number of devices utilized;
each device receives a disjoint subset of the dataset and no samples are
shuffled or exchanged between compute devices outside of the gradient
averaging. Caffe frequently uses a database in LMDB format for its
datasets, however this format cannot be used on remote (network)
filesystems or simultaneously between more than one process on the same
host. Caffe mitigates
this issue when using more than one GPU on the same host by using a
single I/O reading thread and a round-robin deal of the samples to
device-specific queues. Our implementations mitigate this issue by first
converting an LMDB database into a netCDF file~\citep{netcdf}. netCDF
files can be read and partitioned using parallel MPI-IO via the parallel
netCDF library~\citep{pnetcdf}.

\subsection{MPI Implementation Details}
For single-node GPU computation, using one or more GPU devices in a
single host, Caffe provides a means of allocating one contiguous buffer
to hold the data for the weights and biases and a second buffer to hold
the gradients for each. We extended this approach for CPU hosts. A
single contiguous buffer allows the non-layer-wise, i.e., network-wise
gradient averages to be performed using a single MPI reduction
operation. The layer-wise implementations require one MPI reduction
operation per network parameter. There is a fixed cost to start a
communication primitive regardless of how much data is communicated. It
is sometimes beneficial to aggregate otherwise many small communication
requests into a larger one.

Although Caffe provides a way of utilizing all GPUs within the host, it
does not currently leverage NVIDIA's NCCL package~\citep{NCCL} for
optimized, high-bandwidth collective communication routines. We
used the NCCL equivalent to the MPI all reduction to sum gradients
across GPU devices on the DGX-1 platform. 



==> text/impl.tex <==
\subsection{Implementation Details}
\subsubsection{Multi-GPU Implementation Details}
Multiple GPUs on a compute node are commonplace in modern systems such as
NVIDIA DGX-1 architecture.  We leverage the
NVIDIA-Caffe~\cite{caffe-nvidia}, which uses NVIDIA Collective Communication Library
(NCCL)~\cite{NCCL} and its high performance implementations of
all-to-all reduction and other collective communication primitives. 

\subsubsection{Multi-Node Xeon Implementation Details}
Our distributed memory implementation of SGD for Intel Xeon based multi-core systems is built on
MPI~\cite{mpi1,mpi2}.  Similar implementations have been proposed by other approaches
such as FireCaffe and S-Caffe~\cite{firecaffe,scaffe}.  However, unlike FireCaffe, we maintain
strict equivalence to the default sequential SGD  by conducting an
\texttt{MPI\_Allreduce} at the end of each batch. FireCaffe instead
communicates once every few batches and hence does not maintain the equivalance. 
For implementation on Xeon systems, we use Intel-Caffe as the baseline.
While Intel-Caffe also provides a distributed SGD
implementation, it uses a parameter server paradigm, and hence it is not equivalent to the default SGD algorithm.
%Hence, we extend single node Intel-Caffe for distributed memory implementation
%using MPI. 

\subsubsection{Multi-Node, Multi-GPU Implementation Details}
For multi-node multi-GPU systems (where each node may have one or more GPUs
such as presented in section~\ref{sec:exp}), we use NCCL based all-to-all
reduction within a node, and MPI implementation of all-to-all reduction across
multiple compute nodes. The publicly available multi-node implementations of
Caffe -- such as OSU-Caffe -- are not optimized for NCCL, and conduct an
all-to-all reduction of gradients during back-propagation itself. Other
implementations such as Inspur Caffe, MXNet provide parameter-server based
implementation.  Hence, we extend NVIDIA-Caffe which contains NCCL optimization
and leverage it for implementing SGD, Asynchronous SGD and GossipGraD.



==> text/intro_vishnu.tex <==
\section{Introduction}
\label{sec:intro}
Deep Learning (DL) algorithms conduct non-parametric modeling by emulating the
computational structure of a mammalian brain.  By using {\em layers} of {\em neurons} 
interconnected with each other, DL algorithms are able to conduct a
series of non-linear transformations. These properties have been a critical for
success of DL implementations on several machine learning and data mining
(MLDM) tasks such as clustering, classification, anomaly detection and
regression. Several domains such as computer vision, high energy physics,
quantum chemistry and climate have demonstrated significant improvement in
accuracy using DL algorithms. Open source implementations such as Caffe,
Theano, Torch and TensorFlow have further improved the adoption of DL
implementations across new fields.  At the same time, volume of data produced by simulations, experiments and
handheld devices continues to grow rapidly. An important technique for DL
analysis on this rapidly growing data is by leveraging massive parallelism
available with supercomputers, and cloud computing systems. Several researchers have proposed solutions for designing distributed DL algorithms [cite like 15 things].


==> text/motivation.tex <==



==> text/palagrad_proof.tex <==
%\documentclass{article}
%\usepackage{amsthm}
%\newtheorem{theorem}{Theorem}
%\begin{document}
\section{Proof of Equivalence to Batch Gradient Descent}
\label{sec:proof}
\begin{theorem}
The PALaGrad algorithm is equivalent to batch gradient descent.
\end{theorem}

\begin{proof}
The key observation is that the gradient updates are computed independently for each sample in both cases, before averaging and application.

Let $\nabla_i^\ell$ indicate the gradients of the $i$th sample in the batch of $n$ samples for layer $\ell$.  In batch gradient descent, the computation of the total gradients $\nabla^\ell$ for each layer occur either simultaneously or sequentially, but only after all $\nabla_i^\ell$ have been computed is $\nabla^\ell = \frac{1}{n}\sum_{i=1}^n \nabla^\ell_i$ and then applied as a weight update.

In PALaGrad, each node has $k$ samples, so if there are $r$ nodes we have $n=kr$.  If $L$ is the index of the last layer, then first, we compute $\nabla_i^L$ for all $i$.  Then, simultaneously, these gradients are passed within each node to compute $\nabla_i^{L-1}$ and the global gradient $\nabla^L=\frac{1}{n}\sum_{i=1}^n \nabla_i^L$ is computed and applied.  As $\nabla_i^{L-1}$ only depends on $\nabla_i^L$ for the same $i$, the values of the $\nabla_i^{L-1}$ agree for batch gradient descent and PALaGrad.  Furthermore, when these are averaged, the global gradients agree as well.

By induction, every global gradient $\nabla^\ell$ for PALaGrad and batch gradient descent will agree.  As PALaGrad waits for all gradients to be computed before moving on to the next batch, this implies that, if the weights of the network trained with each method agree before a batch, they will agree after the batch, which demonstrates the equivalence.
\end{proof}
%\end{document}


==> text/perf.tex <==
\section{Performance Evaluation}
\label{sec:exp} 
In this section, we present an in-depth evaluation of AGD, GossipGraD and its
associated heuristics using well-studied neural network topologies and
ImageNet-1K dataset. Table~\ref{table:arch} provides a description of the
architectures used for performance evaluation.  Table~\ref{table:datasets}
provides a brief description of the datasets used for performance evaluation.
Table~\ref{table:heur_desc} provides a description of the heuristics.

\begin{table*}[!htbp] 
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
				\hline
				Name  & CPU (\#cores) & \# GPUs/node & Baseline & Network & MPI &  Nodes & \#cores & \# GPUs\\
				\hline 
				\bf{Pascal} & Power8 (20) & NVIDIA Pascal P100 (4) & NVIDIA-Caffe\cite{caffe-nvidia} & NVLink, IB-EDR  & IBM MPI & 32 & N/A & 128\\
%				\bf{DGX-1} & Haswell (16) & Pascal (8) & nVIDIA-Caffe\cite{caffe-nvidia} & NVLink & N/A & 5.1 &  8 & 1 & 40\\
				\bf{SB} & Sandybridge (16) & N/A & Intel-Caffe\cite{caffe-intel} & IB-FDR & IMPI 5.1.2 &  128 & 2048 & N/A\\
				\hline
		\end{tabular}\\  
		\caption{Description of System Architectures.}
		\label{table:arch}  
\end{table*}

\begin{table*}[!t] 
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Dataset  & Neural Network     & Description & Training Samples & Validation Samples & Image Size            & Classes \\
\hline 
ImageNet~\cite{ILSVRC15} & AlexNet~\cite{NIPS2012_4824} & Diverse Images & 1281167          & 50000              & $256\times256\times3$  & 1000 \\
ImageNet & GoogLeNet~\cite{43022} & Diverse Images & 1281167          & 50000              & $256\times256\times3$ & 1000 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{A Description of datasets and associated neural network topologies}
\label{table:datasets}  
\end{table*}

\begin{table*}[!t] 
		\centering
        \small
		\begin{tabular}{|c|c|c|l|}
				\hline
				Name  & Type  & Implemented & Description of DL Algorithm and Implementation\\
				\hline
				SGD & Stochastic Gradient Descent (GD) & Yes & Implements GD by dividing batch and all-to-all reduction. \\
				AGD & Asynchronous GD & Yes & Implements SGD by asynchronous layer-wise communication. \\
				BaG & Batch-wise Asynchronous Gossip GD & Yes & Implements batch-wise AGD using Gossip Protocol \\
				BaRG & Batch-wise Asynchronous Gossip GD with Rotation & Yes & Implements batch-wise AGD using Gossip and Rotation \\
				LaG & Layer-wise Asynchronous Gossip GD & Yes & Implements layer-wise AGD using Gossip Protocol \\
				LaRG & Layer-wise Asynchronous Gossip GD with Rotation & Yes & Implements layer-wise AGD using Gossip and Rotation \\
				\hline
		\end{tabular}\\  
		\caption{Description of Approaches. We implement six approaches and evaluate them on GPU and CPU systems. }
		\label{table:heur_desc}  
\end{table*}

\subsection{Baseline Performance}
We first provide performance comparisons between a single compute node of SB
(please refer Table~\ref{table:arch}) and a single Pascal GPU. We observe that
a single Pascal P100 is 13.66x faster than SB on AlexNet and 7.76x faster on
GoogLeNet using a mini-batch size of 16. AlexNet has $\approx$ 12x more weights
-- which implies that the communication volume of AlexNet is significantly
higher than GoogLeNet.

\subsection{Performance Evaluation of MNIST and CIFAR10 Datasets}


\subsection{Performance Comparison of SGD and AGD}
Figure~\ref{fig:SGDvAGD_SB} shows the performance comparison of AlexNet on
ImageNet-1K with SB architecture using up to 64 compute nodes. We use one
process per compute node. 
%and strong scaling (a global batch size of 256 samples),
%as used by other researchers~\cite{matex,das:arxiv16,scaffe}.  
We observe that
AGD is consistently faster than SGD, because it is able to overlap
communication with the compute of back-propagation (section~\ref{sec:asyncgd}),
while SGD executes an all-to-all reduction after the back-propagation step --
providing no opportunity for overlap.  

\subsubsection{Lessons Learned}
AGD is consistently faster than SGD under the metric of batches per second.
Since AGD is theoretically equivalent to SGD -- we consider AGD as the baseline
for performance and accuracy comparisons for rest of the paper.
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/sgd_vs_agd.pdf}
\caption{Batches per second of AGD in comparison to SGD on SB
architecture using AlexNet up to 64 nodes (1024 cores)}
\label{fig:SGDvAGD_SB}
\end{figure}

\begin{figure*}[htbp]
\begin{minipage}[t]{\columnwidth}
\centering
\includegraphics[width=\columnwidth]{./fig/AGDvBaG_SB.pdf}
\caption{Batch updates/second of BaG in comparison to AGD on SB architecture using AlexNet up to 128 nodes}
\label{fig:AGDvBaG_SB}
\end{minipage}
\hfill
\centering
\begin{minipage}[t]{\columnwidth}
\centering
\includegraphics[width=\columnwidth]{./fig/AGDvBaG_P1.pdf}
\caption{Batch updates/second of BaG in comparison to AGD on Pascal architecture using GoogLeNet up to 128 GPUs}
\label{fig:AGDvBaG_P1}
\end{minipage}
\end{figure*}

\subsection{Performance Comparisons of AGD with Asynchronous GossipGraD}
Figures~\ref{fig:AGDvBaG_SB} and~\ref{fig:AGDvBaG_P1} show the performance
comparison of AGD with Batch-wise Asynchronous GossipGraD (BaG in
Table~\ref{table:heur_desc}). We use 1 MPI process per compute node on SB
architecture and a batch size of sixteen per process for weak scaling, as
suggested in several evaluations for scaling out DL
implementations~\cite{matex, scaffe, li:nips14,das:arxiv16}.  On SB
architecture, we observe that BaG is consistently faster than AGD ($\approx$
1.4x speedup), since the communication complexity reduces from $\Theta(\log(p))$
to $O(1)$. 

Figure~\ref{fig:AGDvBaG_P1} shows the results for GoogLeNet on ImageNet-1K
dataset using up to 128 GPUs (32 nodes x 4 GPUs/node).  GoogLeNet has 18x number
of layers than AlexNet, and much more computationally expensive than AlexNet,
and requires only a small fraction of communication volume in comparison to
AlexNet.  However, even with this property and using a weak-scaling mode (fixed
work/process), AGD is unable to scale well beyond 8 GPUs, and observes a sharp
reduction in batch updates/second thereafter. Upon further investigation, we
observe that the majority of time is spent waiting for asynchronous all-to-all
reduction(s) from previous layers to complete under this configuration. Since
P100 is 13.66x faster than SB on one compute node, communication becomes
the dominating factor quickly (4 GPU case use only NVLINK, since they are co-located on
one node).  

\ABHINAV{Can we get some MPI numbers here}
From performance perspective, we observed that other GossipGraD approaches such
as BaRG, LaG, and LaRG performed similarly to BaG. This is expected because
these approaches are equivalent in terms of communication complexity to BaG. Hence, performance results for these approaches are not shown.

\subsubsection{Lessons Learned}
We observe that while the performance benefits of GossipGraD on SB architecture
are modest, the advantages on Pascal are significant ({\bf 15x} speedup from
AGD both using 128 GPUs, and {\bf 108x} for GossipGraD in comparison to 1 GPU). The Pascal GPUs which reduce the computation time drastically
highlight the impact of gossip communication protocol, even though Pascal uses
the InfiniBand EDR -- the fastest available InfiniBand communication network.  
This result highlights the clear advantage of GossipGraD over AGD.

However, it is equally important to consider the loss and accuracy comparisons
of AGD and GossipGraD. That is the focus of the next section.

\begin{figure*}[htbp]
\begin{minipage}[t]{\columnwidth}
\centering
		\includegraphics[width=\columnwidth]{./fig/all_losses.pdf}
		\caption{Smoothed Loss curves for hypercube and dissemination variants of BaG, BaRG, LaG and LaRG to AGD for GoogLeNet on 32 GPUs}
		\label{fig:HypvDiss}
\end{minipage}
\hfill
\centering
\begin{minipage}[t]{\columnwidth}
\centering
		\includegraphics[width=\columnwidth]{./fig/cascade_acc.pdf}
		\caption{Accuracy Comparisons on AlexNet using SB Architecture as a function of batch updates.}
		\label{fig:AGDvBaG_SB_Acc}
\end{minipage}
\end{figure*}
\subsection{Loss Curve Comparisons}
%of AGD and GossipGraD with hypercube and dissemination}
Figure~\ref{fig:HypvDiss} shows the comparison of hypercube and dissemination
variants of BaG, BaRG, LaG and LaRG in comparison to AGD.  Firstly, we observe
that with an exception of LaG, losses continue to decrease for other GossipGraD
variants. A few of these variants observe similar loss as AGD. Batch-wise
implementations -- with (BaRG) and without (BaG) rotation -- provided similar
loss.  Upon further investigation, we observed that the gradient updates
provided by most samples in ImageNet-1K are roughly similar for both these
approaches. Hence, both approaches provided similar loss pattern.  Yet,
rotation based approach is suitable in general to other datasets -- since it has
the ability to diffuse the results to a wider set of compute nodes without
incurring additional time-complexity.

Upon further investigation of LaG loss, we pin-pointed the behavior to
multiple layers receiving updates from the same partner. For example with
GoogLeNet on 128 GPUs, the partners were repeated after back-propagation on 7
($\log(128) = 7)$ layers.  This de-stabilized the model weights that existed
between the layers updated by the same partner.  As a result, loss pattern for
LaG was sub-optimal. We also observed that dissemination/hypercube algorithm
based partner selection did not affect the loss chart. Since
hypercube based partner selection ensured that at least two nodes averaged their
models at one step (batch/layer), we use hypercube based partner selection for rest of the
paper.

\subsection{Accuracy Comparisons}
Figure~\ref{fig:AGDvBaG_SB_Acc} shows the accuracy comparisons between AGD and
GossipGraD (BaG) from 16 nodes to 128 compute nodes on SB architecture. We
expect similar charts for the Pascal architecture, since implementations are
algorithmically equivalent and architecture independent. 

We use weak-scaling mode (16 mini-batch for each process) and execute 16, 32
node execution for 6 hours each, while execute 64 and 128 node for 4 hours
each.  We make the following observations: 1) weak-scaling reduces the time-to-solution
for both AGD and BaG -- hence it is a viable approach for scaling DL
implementations, 2) BaG starts with a lower accuracy (since only a little
diffusion has been conducted to that point), but starts to converge -- and in
some cases out-performs the AGD implementation under accuracy, 3) GossipGraD is able to reduce
time-to-solution to a user-defined accuracy point in comparison to AGD.

Figure~\ref{fig:top5final} shows the comparison of GossipGraD and AGD using 128
Pascal GPUs on top-5 accuracy.  We show a snippet of overall batches to
demonstrate the difference between AGD and GossipGraD. As observed earlier,
GossipGraD (in this specific case BaG) is 15x faster than AGD in terms of batch
updates/second.  However, we observed that GossipGraD is also better/similar in terms
of observed accuracy after same number of batch updates. Up on further
investigation, we pointed that on 128 GPUs, the effective batch size for AGD is
2048 (16 mini batch on each GPU). A smaller mini-batch reduced the scalability
dramatically. However, even after using Krizhevsky's suggestion of learning
rate modification~\cite{oneweirdtrick}, a larger batch diluted the gradients
for AGD. However, GossipGraD received an unexpected advantage -- not only in
terms of time complexity -- but lesser dilution in terms of observed accuracy,
since when two processes combined their gradients, the effective batch size was 32 -- which is the original suggested batch size for GoogLeNet.


\subsection{Insight and Discussion}
We expected an improvement in time-complexity for GossipGraD since the
communication reduced from $\log(p)$ to $O(1)$. However, in several cases, we
also observed an improvement in the accuracy -- which was a surprising result.
Upon investigation, we pin-pointed that SGD, AGD and GossipGraD requires
setting up several hyper-parameters, which affect the loss and accuracy charts.
As suggested by Krizhevsky {\em et al.}~\cite{oneweirdtrick}, we multiplied the
learning rate by $\sqrt{2}$, as number of compute nodes were doubled. However,
as Krizhevsky {\em et al.} pointed out, this modification is not optimal --
since it does not provide similar loss as strong scaling. By increasing the
batch size, the gradients get diluted for AGD, even after the learning rate
modification.  At the same time, strong scaling beyond a few compute nodes is
not possible -- since there is insufficient work per compute node or device.
However, GossipGraD addresses this problem in a simple way. At any step,
GossipGraD combines the gradients of only two processes. Hence, the gradients
are not diluted similarly as AGD.  As a result, even though GossipGraD might
trail AGD during the first set of batch updates, it catches up quickly and
surpasses the accuracy provided by AGD. This makes GossipGraD suitable on performance and accuracy metrics.

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.67\columnwidth]{./fig/loss3final.pdf}
%\caption{Batches per second of AGD in comparison to SGD on SB
%architecture using AlexNet up to 64 nodes (1024 cores)}
%\label{fig:loss3final}
%\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/top5final.pdf}
\caption{top-5 accuracy comparison between AGD and GossipGraD using GoogLeNet on 128 Pascal GPUs}
\label{fig:top5final}
\end{figure}




==> text/perf_save.tex <==
\section{Performance Evaluation}
\label{sec:exp} 
In this section, we present an in-depth evaluation of GossipGraD and its
associated heuristics using datasets such as MNIST, CIFAR10 and well-studied neural network topologies and
ImageNet-1K dataset. The table~\ref{table:arch} provides a description of the
architectures used for performance evaluation.  Table~\ref{table:datasets}
provides a brief description of the datasets used for performance evaluation.
Table~\ref{table:heur_desc} provides a description of the heuristics.

\begin{table*}[!htbp] 
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
				\hline
				Name  & CPU (\#cores) & \# GPUs/node & Baseline & Network & MPI &  Nodes & \#cores & \# GPUs\\
				\hline 
				\bf{Pascal} & Power8 (20) & NVIDIA Pascal P100 (4) & NVIDIA-Caffe\cite{caffe-nvidia} & NVLink, IB-EDR  & IBM MPI & 32 & N/A & 128\\
%				\bf{DGX-1} & Haswell (16) & Pascal (8) & nVIDIA-Caffe\cite{caffe-nvidia} & NVLink & N/A & 5.1 &  8 & 1 & 40\\
				\bf{Titan} & Opteron (16) & NVIDIA K20 (1) & NVIDIA-Caffe\cite{caffe-nvidia} & Gemini & Cray MPICH &   512 & N/A & 512\\
				\bf{SB} & Sandybridge (16) & N/A & Intel-Caffe\cite{caffe-intel} & IB-FDR & IMPI 5.1.2 &  128 & 2048 & N/A\\
				\hline
		\end{tabular}\\  
		\caption{A description of system architecture and associated software}
		\label{table:arch}  
\end{table*}

\begin{table*}[!t] 
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Dataset  & Neural Network     & Description & Training Samples & Validation Samples & Image Size            & Classes\\
\hline 
MNIST~\cite{mnistlecun}    & LeNet-3~\cite{lecun1998gradient} & Handwritten Digits & 60000            & 10000          &     $28 \times28$ & 10        \\
CIFAR-10~\cite{Krizhevsky09learningmultiple} & Caffe-default  & Small Images & 60000            & 10000              & $32 \times32\times3$  & 10  \\
ImageNet & GoogLeNet~\cite{43022} & Diverse Images & 1281167          & 50000              & $256\times256\times3$ & 1000  \\
ImageNet & ResNet~\cite{he2016deep} & Diverse Images & 1281167          & 50000              & $256\times256\times3$ & 1000\\
\hline
\end{tabular}
\end{adjustbox}
\caption{A description of datasets and associated neural network topolgies}
\label{table:datasets}  
\end{table*}

\begin{table*}[!t] 
		\centering
        \small
		\begin{tabular}{|c|c|c|l|}
				\hline
				Name  & Type  & Implemented & Description of DL Algorithm and Implementation\\
				\hline
				SGD & Stochastic Gradient Descent (GD) & Yes & Implements GD by dividing batch and all-to-all reduction. \\
				AGD & Asynchronous GD & Yes & Implements SGD by asynchronous layer-wise communication. \\
				%BaG & Batch-wise Asynchronous Gossip GD & Yes & Implements batch-wise AGD using Gossip Protocol \\
				BaG & Batch-wise Gossip GD with Rotation of partners and samples& Yes & Implements batch-wise AGD using Gossip and Rotation of Samples \\
				%LaG & Layer-wise Asynchronous Gossip GD & Yes & Implements layer-wise AGD using Gossip Protocol \\
				%LaRG & Layer-wise Asynchronous Gossip GD with Rotation & Yes & Implements layer-wise AGD using Gossip and Rotation \\
				\hline
		\end{tabular}\\  
		\caption{A description of GossipGraD Approaches. We implement these approaches and evaluate them on GPU and CPU systems.}
		\label{table:heur_desc}  
\end{table*}

\subsection{Baseline Performance}
We first provide performance comparisons between a single compute node of SB
(please refer Table~\ref{table:arch}) and a single Pascal GPU. We observe that
a single Pascal P100 is 13.66x faster than SB on AlexNet and 7.76x faster on
GoogLeNet using a mini-batch size of 16. AlexNet has $\approx$ 12x more weights
-- which implies that the communication volume of AlexNet is significantly
higher than GoogLeNet.

\subsection{Performance Comparison of SGD and AGD}
Figure~\ref{fig:SGDvAGD_SB} shows the performance comparison of AlexNet on
ImageNet-1K with SB architecture using up to 64 compute nodes. We use one
process per compute node. 
%and strong scaling (a global batch size of 256 samples),
%as used by other researchers~\cite{matex,das:arxiv16,scaffe}.  
We observe that
AGD is consistently faster than SGD, because it is able to overlap
communication with the compute of back-propagation (section~\ref{sec:asyncgd}),
while SGD executes an all-to-all reduction after the back-propagation step --
providing no opportunity for overlap.  

\subsubsection{Lessons Learned}
AGD is consistently faster than SGD under the metric of batches per second.
Since AGD is theoretically equivalent to SGD -- we consider AGD as the baseline
for performance and accuracy comparisons for rest of the paper.
\begin{figure*}[htbp]
%\begin{figure}[htbp]
\begin{minipage}[t]{0.66\columnwidth}
\centering
\includegraphics[width=\columnwidth]{./fig/sgd_vs_agd.pdf}
\caption{Batch updates per second of AGD in comparison to SGD on SB
architecture using AlexNet up to 64 nodes (1024 cores)}
\label{fig:SGDvAGD_SB}
\end{minipage}
\hfill
%\end{figure}
\begin{minipage}[t]{0.66\columnwidth}
\centering
\includegraphics[width=\columnwidth]{./fig/AGDvBaG_SB.pdf}
\caption{Batch updates/second of BaG in comparison to AGD on SB architecture using AlexNet up to 128 nodes}
\label{fig:AGDvBaG_SB}
\end{minipage}
\hfill
\centering
\begin{minipage}[t]{0.66\columnwidth}
\centering
\includegraphics[width=\columnwidth]{./fig/AGDvBaG_P1.pdf}
\caption{Batch updates/second of BaG in comparison to AGD on Pascal architecture using GoogLeNet up to 128 GPUs}
\label{fig:AGDvBaG_P1}
\end{minipage}
\end{figure*}

\subsection{Performance Evaluation on MNIST and CIFAR10}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/MNIST.pdf}
\label{fig:MNIST}
\caption{MNIST caption TODO}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/CIFAR10.pdf}
\label{fig:CIFAR10}
\caption{CIFAR10 caption TODO}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/MNIST-speedup.pdf}
\label{fig:MNIST-speedup}
\caption{MNIST caption TODO}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/CIFAR-speedup.pdf}
\label{fig:CIFAR10-speedup}
\caption{CIFAR10 caption TODO}
\end{figure}

\begin{table*}[!t] 
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
Sync Method & Average +- StdDev & Min & Max \\
\hline 
SGD-CPU & 64.0201 +- 11.2882 & 24.7097 & 79.8722 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{MNIST Performance}
\label{table:mnist_perf}  
\end{table*}

\subsection{Performance Comparisons of AGD with Asynchronous GossipGraD}
\ABHINAV{alexnet mini-batch 16 2.17415 iter/s, 9.199s/20 iter
alexnet mini-batch 256 0.260794 iter/s, 76.689s/20 iter
gnet mini 16 1.1556 iter/s, 34.614s/40 iter
gnet mini 32 0.732869 iter/s, 54.58s/40 iter
Pascal:
alexnet batch 256 3.52671 iter/s, 5.67101s/20 iter
alexnet batch 16 29.4769 iter/s, 0.678498s/20 iter
gnet batch 16 8.73342 iter/s, 4.58011s/40 iter
gnet batch 32 5.68189 iter/s, 7.03991s/40 iter
}

Figures~\ref{fig:AGDvBaG_SB} and~\ref{fig:AGDvBaG_P1} show the performance
comparison of AGD with Batch-wise Asynchronous GossipGraD (BaG in
Table~\ref{table:heur_desc}). We use 1 MPI process per compute node on SB
architecture and a batch size of sixteen per process for weak scaling, as
suggested in several evaluations for scaling out DL
implementations~\cite{matex, scaffe, li:nips14,das:arxiv16}.  On SB
architecture, we observe that BaG is consistently faster than AGD ($\approx$
1.4x speedup), since the communication complexity reduces from $\Theta(\log(p))$
to $O(1)$. 

Figure~\ref{fig:AGDvBaG_P1} shows the results for GoogLeNet on ImageNet-1K
dataset using up to 128 GPUs (32 nodes x 4 GPUs/node).  GoogLeNet has 18x number
of layers than AlexNet, and much more computationally expensive than AlexNet,
and requires only a small fraction of communication volume in comparison to
AlexNet.  However, even with this property and using a weak-scaling mode (fixed
work/process), AGD is unable to scale well beyond 8 GPUs, and observes a sharp
reduction in batch updates/second thereafter. Upon further investigation, we
observe that the majority of time is spent waiting for asynchronous all-to-all
reduction(s) from previous layers to complete under this configuration. Since
P100 is 13.66x faster than SB on one compute node, communication becomes
the dominating factor quickly (4 GPU case use only NVLINK, since they are co-located on
one node).  

\ABHINAV{Can we get some MPI numbers here}
From performance perspective, we observed that other GossipGraD approaches such
as BaRG, LaG, and LaRG performed similarly to BaG. This is expected because
these approaches are equivalent in terms of communication complexity to BaG. Hence, performance results for these approaches are not shown.

\subsubsection{Lessons Learned}
We observe that while the performance benefits of GossipGraD on SB architecture
are modest, the advantages on Pascal are significant ({\bf 15x} speedup from
AGD both using 128 GPUs, and {\bf 108x} for GossipGraD in comparison to 1 GPU). The Pascal GPUs which reduce the computation time drastically
highlight the impact of gossip communication protocol, even though Pascal uses
the InfiniBand EDR -- the fastest available InfiniBand communication network.  
This result highlights the clear advantage of GossipGraD over AGD.

However, it is equally important to consider the loss and accuracy comparisons
of AGD and GossipGraD. That is the focus of the next section.

\begin{figure*}[htbp]
\begin{minipage}[t]{\columnwidth}
\centering
		\includegraphics[width=\columnwidth]{./fig/all_losses.pdf}
		\caption{Smoothed Loss curves for hypercube and dissemination variants of BaG, BaRG, LaG and LaRG to AGD for GoogLeNet on 32 GPUs}
		\label{fig:HypvDiss}
\end{minipage}
\hfill
\centering
\begin{minipage}[t]{\columnwidth}
\centering
		\includegraphics[width=\columnwidth]{./fig/cascade_acc.pdf}
		\caption{Accuracy Comparisons on AlexNet using SB Architecture as a function of batch updates.}
		\label{fig:AGDvBaG_SB_Acc}
\end{minipage}
\end{figure*}
\subsection{Loss Curve Comparisons}
%of AGD and GossipGraD with hypercube and dissemination}
Figure~\ref{fig:HypvDiss} shows the comparison of hypercube and dissemination
variants of BaG, BaRG, LaG and LaRG in comparison to AGD.  Firstly, we observe
that with an exception of LaG, losses continue to decrease for other GossipGraD
variants. A few of these variants observe similar loss as AGD. Batch-wise
implementations -- with (BaRG) and without (BaG) rotation -- provided similar
loss.  Upon further investigation, we observed that the gradient updates
provided by most samples in ImageNet-1K are roughly similar for both these
approaches. Hence, both approaches provided similar loss pattern.  Yet,
rotation based approach is suitable in general to other datasets -- since it has
the ability to diffuse the results to a wider set of compute nodes without
incurring additional time-complexity.

Upon further investigation of LaG loss, we pin-pointed the behavior to
multiple layers receiving updates from the same partner. For example with
GoogLeNet on 128 GPUs, the partners were repeated after back-propagation on 7
($\log(128) = 7)$ layers.  This de-stabilized the model weights that existed
between the layers updated by the same partner.  As a result, loss pattern for
LaG was sub-optimal. We also observed that dissemination/hypercube algorithm
based partner selection did not affect the loss chart. Since
hypercube based partner selection ensured that at least two nodes averaged their
models at one step (batch/layer), we use hypercube based partner selection for rest of the
paper.

\subsection{Accuracy Comparisons}
Figure~\ref{fig:AGDvBaG_SB_Acc} shows the accuracy comparisons between AGD and
GossipGraD (BaG) from 16 nodes to 128 compute nodes on SB architecture. We
expect similar charts for the Pascal architecture, since implementations are
algorithmically equivalent and architecture independent. 

We use weak-scaling mode (16 mini-batch for each process) and execute 16, 32
node execution for 6 hours each, while execute 64 and 128 node for 4 hours
each.  We make the following observations: 1) weak-scaling reduces the time-to-solution
for both AGD and BaG -- hence it is a viable approach for scaling DL
implementations, 2) BaG starts with a lower accuracy (since only a little
diffusion has been conducted to that point), but starts to converge -- and in
some cases out-performs the AGD implementation under accuracy, 3) GossipGraD is able to reduce
time-to-solution to a user-defined accuracy point in comparison to AGD.

Figure~\ref{fig:top5final} shows the comparison of GossipGraD and AGD using 128
Pascal GPUs on top-5 accuracy.  We show a snippet of overall batches to
demonstrate the difference between AGD and GossipGraD. As observed earlier,
GossipGraD (in this specific case BaG) is 15x faster than AGD in terms of batch
updates/second.  However, we observed that GossipGraD is also better/similar in terms
of observed accuracy after same number of batch updates. Up on further
investigation, we pointed that on 128 GPUs, the effective batch size for AGD is
2048 (16 mini batch on each GPU). A smaller mini-batch reduced the scalability
dramatically. However, even after using Krizhevsky's suggestion of learning
rate modification~\cite{oneweirdtrick}, a larger batch diluted the gradients
for AGD. However, GossipGraD received an unexpected advantage -- not only in
terms of time complexity -- but lesser dilution in terms of observed accuracy,
since when two processes combined their gradients, the effective batch size was 32 -- which is the original suggested batch size for GoogLeNet.


\subsection{Insight and Discussion}
We expected an improvement in time-complexity for GossipGraD since the
communication reduced from $\log(p)$ to $O(1)$. However, in several cases, we
also observed an improvement in the accuracy -- which was a surprising result.
Upon investigation, we pin-pointed that SGD, AGD and GossipGraD requires
setting up several hyper-parameters, which affect the loss and accuracy charts.
As suggested by Krizhevsky {\em et al.}~\cite{oneweirdtrick}, we multiplied the
learning rate by $\sqrt{2}$, as number of compute nodes were doubled. However,
as Krizhevsky {\em et al.} pointed out, this modification is not optimal --
since it does not provide similar loss as strong scaling. By increasing the
batch size, the gradients get diluted for AGD, even after the learning rate
modification.  At the same time, strong scaling beyond a few compute nodes is
not possible -- since there is insufficient work per compute node or device.
However, GossipGraD addresses this problem in a simple way. At any step,
GossipGraD combines the gradients of only two processes. Hence, the gradients
are not diluted similarly as AGD.  As a result, even though GossipGraD might
trail AGD during the first set of batch updates, it catches up quickly and
surpasses the accuracy provided by AGD. This makes GossipGraD suitable on performance and accuracy metrics.

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.67\columnwidth]{./fig/loss3final.pdf}
%\caption{Batches per second of AGD in comparison to SGD on SB
%architecture using AlexNet up to 64 nodes (1024 cores)}
%\label{fig:loss3final}
%\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/top5final.pdf}
\caption{top-5 accuracy comparison between AGD and GossipGraD using GoogLeNet on 128 Pascal GPUs}
\label{fig:top5final}
\end{figure}




==> text/perf_yinyang_save.tex <==
\section{Performance Evaluation}
\label{sec:exp} 
In this section, we present a detailed performance evaluation of proposed YinYang heuristics on several CPU and GPU Clusters, including recently proposed DGX-1 architecture. Table~\ref{table:arch} shows the hardware and software details of our systems. Table~\ref{table:heur_desc} shows a description of heuristics that we have implemented. Table~\ref{table:datasets} provides an overview of datasets, the associated neural networks and a summary of results.

\begin{table*}[!htbp] 
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
				\hline
				Name  & CPU (\#cores) & GPU & Baseline Caffe & Network & MPI & cuDNN & CUDA & Nodes & \#cores\\
				\hline 
				\bf{DGX-1} & Haswell (16) & Pascal (8) & nVIDIA-Caffe & N/A & N/A & 4.5 &  8 & 1 & 40\\
				\bf{K40} & Haswell (20) & K40 & BVLC-Caffe & IB & OpenMPI 1.8.3 & 4 &  7.5 & 8 & 160\\
				\bf{Has} & Haswell (20) & N/A & Intel-Caffe & IB & OpenMPI 1.8.3 & N/A &  N/A & 16 & 320\\
				\bf{SB} & Sandybridge (16) & N/A & Intel-Caffe & IB & Intel MPI 5.1.2 & N/A &  N/A & 64 & 1024\\
				\hline
		\end{tabular}\\  
		\caption{Hardware and Software Description. IB (InfiniBand). The
		proposed research extends Baseline-Caffe incorporating
		architecture specific optimizations provided by vendors.}
		\label{table:arch}  
\end{table*}
\begin{table*}[!t] 
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
				\hline
				Name  & Type& Yin/Yang & Description\\
				\hline 
				\bf{Con} & Constant& Yin & Yin process is executed constantly across epochs  \\
				\bf{Temp} & Temporal&Yin & Yin process is executed as a function of epoch  \\
				\bf{None} & Never& Yang & Yang is never executed (at $\infty$)  \\
				\bf{Eon} & Maximum Eon& Yang & The eon length is user-specified   \\
				\bf{Rand} & Random Sample & Yang & Random samples are used for calculating overall error \\
				\bf{CR} & Critical Ratio & Yang & Critical ratio of $\frac{X_{out}}{X}$ falls below threshold \\
				\bf{Valid} & Validation Error & Yang & Error on the validation set increases \\
				\hline
		\end{tabular}\\  
		\caption{Description of Heuristics. All combinations of Yin and
		Yang heuristics such as Con-Valid, Temp-CR are considered}
		\label{table:heur_desc}  
\end{table*}

\begin{table*}[!t] 
		\centering
		\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
				\hline
				Dataset  & Model     & Description & Training Samples & Validation Samples & Image Size            & Classes & Accuracy & Speedup\\
				\hline 
				MNIST~\cite{mnistlecun}    & LeNet-3~\cite{lecun1998gradient} & Handwritten Digits & 60000            & 10000          &     $28 \times28$ & 10        & 0.9938  & 1.45\\
				CIFAR-10~\cite{Krizhevsky09learningmultiple} & Caffe-default  & Small Images & 60000            & 10000              & $32 \times32\times3$  & 10  & 0.7378  & 1.72\\
				ImageNet~\cite{ILSVRC15} & AlexNet~\cite{NIPS2012_4824} & Diverse Images & 1281167          & 50000              & $256\times256\times3$  & 1000 &  0.494 & 1.61\\
				ImageNet & GoogLeNet~\cite{43022} & Diverse Images & 1281167          & 50000              & $256\times256\times3$ & 1000 &  0.55392 & 1.55\\
				\hline
		\end{tabular}
		\end{adjustbox}
		\caption{Datasets and Models evaluated with a Summary of Results}
		\label{table:datasets}  
\end{table*}

%\ABHINAV {colors should be red, orange, green, black and yellow}

\subsection{Baseline Results using MNIST and CIFAR-10}
We use MNIST and CIFAR-10 to perform a sensitivity study for several combinations of heuristics. For MNIST, we use the LeNet-3 network architecture described by LeCun {\em et al.}~\cite{lecun1998gradient}. LeNet-3 consisting of two convolution layers (of 20 and 50 features  each with a max-pooling layer) , followed by a fully connected layer with 500 features.  For CIFAR-10, we use the default network included with Caffe, which consists of three pairs of alternating convolution and max-pooling layers with 32, 32 and 64 features, followed by a fully connected layer with 64 features.

From Table~\ref{table:heuristic_speedups}, we observe that Con-None, a Yin-only
heuristic defined in Table~\ref{table:heur_desc}, provides significant speedup
-- albeit at significant accuracy loss (1.2\% for MNIST, but 7\% for CIFAR),
because Yang is never executed. Con-CR, Temp-CR perform well, but require
manual tuning of CR, which we set to 0.1 for each class. However, its accuracy
is inconsistent, largely because CR removes samples using a ratio independent of
the error in each class. Con-Rand and Temp-Rand are susceptible to sampling --
as reflected in these results, while providing lower speedup as well. Con-Eon
and Temp-Eon provide high accuracy because they periodically execute Yang (we
manually tuned this value to 4). We also observe that validation error based
heuristics -- con-valid and temp-valid provide not only similar accuracy, but
reasonable speedup as well. We contend that this is due to the fact that
validation error acts as a guard from overfitting, which allows Yin to
continue as long as the validation error is not increasing. 
\begin{table}[!t] 
		\centering
		\begin{adjustbox}{max width=\columnwidth}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
				\hline
				Yin      & Yang             & MNIST-Acc & MNIST-Sp. & CIFAR-Acc & CIFAR-Sp.\\
				\hline
				None     & None             & 0.9935 & 1.00 & 0.7231 & 1.00\\
				Con & None             & 0.9803 &10.02 & 0.6536 & 6.67\\
				Con & Eon        & 0.9937 & 1.56 & 0.7416 & 1.40\\
				Con & Rand    & 0.9941 & 1.31 & 0.7317 & 1.52\\
				Con & CR   & 0.9922 & 2.44 & 0.6695 & 1.71\\
				Con & Valid & 0.9938 & 1.45 & 0.7378 & 1.72\\
				Temp& None             & 0.9798 & 7.85 & 0.6851 & 6.51\\
				Temp& Eon          & 0.9930 & 1.78 & 0.7103 & 1.24\\
				Temp& Rand    & 0.9936 & 1.30 & 0.6735 & 1.04\\
				Temp& CR   & 0.9926 & 2.14 & 0.7430 & 1.80\\
				Temp& Valid & 0.9941 & 1.50 & 0.7378 & 1.45\\
				\hline
		\end{tabular} 
		\end{adjustbox}
\caption{Speedups for MNIST and CIFAR-10 on 20 cores with various heuristics on Has system}
\label{table:heuristic_speedups}
\end{table}

We observe that Con-Eon, Con-Valid, Temp-Eon, Temp-Valid perform similar in
accuracy with default case -- while providing significant speedup. We use this
information and conduct a distributed memory evaluation of CIFAR-10 and MNIST
using Has system (as defined in Table~\ref{table:arch}) and 320 cores. These
results are shown in Figures~\ref{fig:mnist} and~\ref{fig:cifar10} for MNIST
and CIFAR-10 respectively. We observe that: 1) At each data point, YinYang
heuristics is equal or better than default implementation 2) Most YinYang
heuristics perform equally well. 

However, the reason to prefer Con-Valid/Temp-Valid over other approaches is the
guard provided by validation set based heuristics, which prevents overfitting
and divergence from a correct solution. Naturally, these approaches result in
no accuracy loss beyond the small error which is introduced as an artifact of
multiple executions. 

\subsection{ImageNet with AlexNet and GoogleNet Neural Network Topology} In
this section, we present results for the ImageNet Large Scale Visualization
Research Challenge (ILSVRC12)~\cite{ILSVRC15}.  We evaluate this dataset on two
distinct neural network topologies,  AlexNet~\cite{NIPS2012_4824} and
GoogLeNet~\cite{43022}. Table~\ref{table:imagenet_speedups} shows the relative
speedup of Con-Valid YinYang heuristic in comparison to the default algorithm
on K40, DGX-1 and SB systems for this comparison, and
Table~\ref{table:alexnet_speedup} shows how this scales for AlexNet on K40
system.

We have a few observations: 1) We achieve 1.37x - 1.61x speedup 2) The accuracy
difference is in the negligible error range subject to different random weight
initializations of neural networks. The speedups are realized on the most
advanced architecture (DGX-1) and a relatively older architecture (K40) --
indicating that we should achieve similar speedups for intermediate
architectures (K80, Titan-X) and upcoming architectures as well.

\begin{figure*}[htbp]
		\begin{minipage}[t]{\columnwidth}
				\centering
\includegraphics[width=\columnwidth]{./fig/MNIST_Scaling_Heuristics3.pdf}
\caption{Relative Speedup to 20 cores for MNIST for selected heuristics
using up to 320 cores}
\label{fig:mnist}
		\end{minipage}
		\centering\hfill
		\begin{minipage}[t]{\columnwidth}
				\centering
\includegraphics[width=\columnwidth]{./fig/CIFAR10_Scaling_Heuristics3.pdf}
\caption{Relative Speedup to 20 cores for CIFAR-10 for selected heuristics
using up to 320 cores}
\label{fig:cifar10}
		\end{minipage}
\end{figure*}
\begin{figure*}[htbp]
		\begin{minipage}[t]{\columnwidth}
				\centering
%\includegraphics[width=\columnwidth]{./fig/alexnet_loss3.pdf}
%\caption{Training loss (YinYang), validation losses for baseline and YinYang approaches using AlexNet}
%\label{fig:alexnet_loss}
\includegraphics[width=\columnwidth]{./fig/alexnet_accuracy.pdf}
\caption{Accuracy for YinYang vs. Default on AlexNet}
\label{fig:alexnet_loss}
		\end{minipage}
		\hfill
		\begin{minipage}[t]{\columnwidth}
				\centering
\includegraphics[width=\columnwidth]{./fig/alexnet_samples3.pdf}
\caption{Number of Active Samples and False-Positives for AlexNet}
\label{fig:alexnet_samples}
		\end{minipage}
\end{figure*}
\begin{figure*}[htbp]
		\begin{minipage}[t]{\columnwidth}
				\centering
\includegraphics[width=\columnwidth]{./fig/googlenet_loss3.pdf}
\caption{Training loss (YinYang), validation losses for baseline and YinYang approaches using GoogleNet}
\label{fig:googlenet_loss}
		\end{minipage}
		\hfill
		\begin{minipage}[t]{\columnwidth}
				\centering
\includegraphics[width=\columnwidth]{./fig/googlenet_samples3.pdf}
\caption{Number of Active Samples and False-Positives for GoogleNet}
\label{fig:googlenet_samples}
		\end{minipage}
\end{figure*}

\begin{table}[!t] 
		\centering
		\begin{adjustbox}{max width=\columnwidth}
		\begin{tabular}{|c|c|c|c|}
				\hline
				Heuristic & 1 GPU& 2 GPU& 4 GPU\\
				\hline
				Default   & 1    & 1.48 & 2.14 \\
				Con-Valid & 1.42 & 2.06 & 3.30 \\
				\hline
		\end{tabular} 
		\end{adjustbox}
\caption{Speedups for AlexNet on GPUs on K40 system, compared to Default on 1 GPU}
\label{table:alexnet_speedup}
\end{table}

\begin{table}[!t]
		\centering
		\begin{adjustbox}{max width=\columnwidth}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
				\hline
				Neural Network & Arch & \#GPUS & Rel. Speedup & Acc.
				Diff.\\
				\hline
				AlexNet & K40 & 4 GPU & 1.61 & $\pm$0.5\\
				AlexNet &  K40 & 8 GPU & 1.44 & $\pm$0.5 \\
				GoogLeNet & K40 & 8 GPU & 1.55 & $\pm$0.4 \\
				AlexNet &  DGX-1 & 8 GPU & 1.37 & $\pm$0.4\\
				GoogLeNet & DGX-1 & 8 GPU & 1.44 & $\pm$0.4\\
				\hline
				 & Arch & \#CPU Cores & Rel. Speedup & Acc.
				Diff.\\
				\hline
				AlexNet & K40 & 400 & 1.50 & $\pm$0.2\\
				AlexNet & SB & 1024 & 1.42 & $\pm$0.3\\
				\hline
		\end{tabular}
		\end{adjustbox}
\caption{Relative Speedup to no-YinYang for K40 and DGX-1 Systems using
ImageNet with AlexNet and GoogleNet}
\label{table:imagenet_speedups}
\end{table}

\subsection{Insight} We have demonstrated through speedups and negligible
accuracy loss that the proposed YinYang heuristics are effective for relatively
straightforward datasets (MNIST, CIFAR-10) and larger, more complex datasets
(ImageNet). Figures~\ref{fig:alexnet_loss} and~\ref{fig:googlenet_loss}
provides insight in the behavior of these heuristics. We observe that the
validation loss -- which is used as method to execute Yang decreases similarly
to the default algorithm. The training loss decreases -- over-fitting as the
size of Yin-phase increases -- but immediately corrects itself, as Yang gets
executed. Figures~\ref{fig:alexnet_samples} and~\ref{fig:googlenet_samples}
show the active samples and false-positives (which are calculated right after
the Yang from the previous epoch is executed). We observe: 1) The number of
active samples is a small fraction of the overall set 2) The number of
false-positives follow a bell-curve pattern, which indicates that they
stabilize by the end of the training -- and hence providing similar accuracy to
the default algorithm.

%\ABHINAV{Need to change legend in Figures 9 and 11: baseline validation loss should be default validation loss, training loss should be YinYang training loss, validation loss should be YinYang validation loss}

\subsection{Discussion}

Overall, YinYang shows a speedup of 1.37x - 1.61x compared to the default
algorithm with no loss of accuracy.  We also observe that although within an
eon the training loss may decrease rapidly, both the validation and training
losses decrease across eons. The last epoch of training is automatically
considered an eon boundary to ensure that all samples are recalled at least
once before the final model is provided for inferencing purposes.
Additionally, the number of false positives decline across eons over the course
of training, indicating that the model is increasingly able to correctly
distinguish between contributing and non-contributing samples.  Furthermore,
the speedup is generally higher the more accurate the model becomes, with
LeNet-3, which achieves $>99\%$ accuracy, having the greatest speedup of all
the models tested.  Finally, Figure~\ref{fig:balance} indicates that
load-balancing is not necessary, as discussed in
Section~\ref{subsec:loadbalance}.

\begin{figure}[hptb]
	\centering
	\includegraphics[width=0.7\columnwidth]{./fig/Alexnet_Sample_Numbers.pdf}
	\caption{Active Samples for each Node for AlexNet Con-Valid on 4 GPUs}
	\label{fig:balance}
\end{figure}

